Be Greedy in Multi-Armed Bandits

The Greedy algorithm is the simplest heuristic in sequential decision problem that carelessly takes the locally optimal choice at each round, disregarding any advantages of exploring and/or information gathering. Theoretically, it is known to sometimes have poor performances, for instance even a linear regret (with respect to the time horizon) in the standard multi-armed bandit problem. On the other hand, this heuristic performs reasonably well in practice and it even has sublinear, and even near-optimal, regret bounds in some very specific linear contextual and Bayesian bandit models. We build on a recent line of work and investigate bandit settings where the number of arms is relatively large and where simple greedy algorithms enjoy highly competitive performance, both in theory and in practice. We first provide a generic worst-case bound on the regret of the Greedy algorithm. When combined with some arms subsampling, we prove that it verifies near-optimal worst-case regret bounds in continuous, infinite and many-armed bandit problems. Moreover, for shorter time spans, the theoretical relative suboptimality of Greedy is even reduced. As a consequence, we subversively claim that for many interesting problems and associated horizons, the best compromise between theoretical guarantees, practical performances and computational burden is definitely to follow the greedy heuristic. We support our claim by many numerical experiments that show significant improvements compared to the state-of-the-art, even for moderately long time horizon.

==> sections/related_work_models.tex <==
\section{Short literature review}
\label{sec:models_review}

In this section, we provide a short literature review on the different bandit models considered in this chapter.

% Continuous-armed bandits
\paragraph{Continuous-armed bandits}
\citet{agrawal1995continuum} introduced the continuous-armed bandit problem with nonparametric regularity assumptions. 
\citet{kleinberg2005nearly} established the lower bound and provide a optimal algorithm up to a sub-logarithmic factor. 
\citet{auer2007improved} improved the previous bound assuming a margin condition. 
\citet{kleinberg2008multi} considered generic metric spaces assuming that the mean-payoff function is Lipschitz with respect to the (known) metric of the space. 
\citet{bubeck2010x} considered generic topological spaces and that the mean-payoff function is locally Lipschitz with respect to a dissimilarity function known to the decision maker. All these works assumed known smoothness parameters; \citet{bubeck2011lipschitz, locatelli2018adaptivity, hadiji2019polynomial} studied the adaptivity to unknown parameters

% Infinite-armed bandits
\paragraph{Infinite-armed bandits}
\citet{berry1997bandit} introduced the infinite-armed bandit problem, they consider a problem consisting of a sequence of $n$ choices from an infinite number of Bernoulli arms, with $n \rightarrow \infty$. The objective is to minimize the long-run failure rate. The Bernoulli parameters are independent observations from a known distribution. 
\citet{bonald2013two} also considered Bernoulli arms but they studied the cumulative regret, focusing on the uniform prior distribution. 
\citet{wang2009algorithms} considered a more general model. In particular they assumed that rewards are uniformly bounded in $[0, 1]$ and that the expected reward of a randomly drawn arm is $\varepsilon$-optimal with probability $\mathcal{O}\left( \varepsilon^\beta \right)$ for some $\beta > 0$.

% Many-armed Bandits
\paragraph{Many-armed bandits}
Models in many-armed bandit problems are more varied.
\citet{teytaud2007anytime} provided an anytime algorithm when the number of arms is large comparatively to the number of time steps.
\citet{wang2017cemab} proposed a cross-entropy based algorithm. They aimed to focus exploration on a small subset of arms. They did not provide theoretical upper bounds.
\citet{chaudhuri2018quantile} introduced a notion of regret with respect to a given quantile fraction $\rho$ of the probability distribution over the expected rewards of arms.
\citet{russo2018satisficing} considered learning a satisficing action and analyze the discounted regret. They propose a Thompson Sampling like algorithm and further studied applications to linear and infinite-armed bandits. The definition of a satisficing action is set by the learner. 
\citet{ou2019semi} proposed a semi-parametric model to formulate expected rewards.
\citet{zhu2020multiple} considered a setting with multiple best/near-optimal arms without making any assumptions about the structure of the bandit instance. Their objective was to design algorithms that can automatically adapt to the unknown hardness of the problem. 

% Linear Bandits
\paragraph{Linear bandits}
The literature on linear bandits is quite large and we refer the reader to \citet{lattimore2018bandit} for an in-depth overview. 
We mention \citet{abbasi2011improved} who proved that an expected regret of $\widetilde{\mathcal{O}}\left( d \sqrt{T} \right)$ can be achieved as long as the means are guaranteed to lie in a bounded interval.
\citet{deshpande2012linear} also considered a linear bandit problem with a dimension that is large relative to the time horizon. They proposed an algorithm that limits exploration and achieves good reward within a short time frame.

% Cascading Bandits
\paragraph{Cascading bandits}
\citet{kveton2015cascading} introduced the cascading bandit model and proposed two algorithms based on UCB and KL-UCB. 
\citet{combes2015learning} proposed an asymptotically optimal algorithm.
\citet{cheung2019thompson} proposed an algorithm based on Thompson Sampling.
\citet{zong2016cascading} considered a linear variant of the model.
\citet{li2016contextual} further considered a contextual setting.

% Mortal Bandits
\paragraph{Mortal bandits}
\citet{chakrabarti2009mortal} introduced the mortal bandit model and proposed an algorithm in which the level of greediness depends on the performance of the best arm available.
%\cite{bnaya2013volatile}?
\citet{traca2019reducing} argued to reduce exploration of dying arms.

% Budgeted Bandits
\paragraph{Budgeted bandits}
\citet{tran2010epsilon} introduced the budgeted bandit problem and proposed an Explore-Then-Commit strategy.
\citet{tran2012knapsack} proposed knapsack-based policies.
\citet{xia2015thompson} proposed a Thomson sampling strategy.
\citet{xia2016budgeted} further extended the problem to continuous random costs
Let us also cite \citet{badanidiyuru2013bandits} who considered a more general framework.

